Toward a realistic model of speech processing in the brain with self-supervised learning

Several deep neural networks have recently been shown to generate activations similar to those of the brain in response to the same input. These algorithms, however, remain largely implausible: they require (1) extraordinarily large amounts of data, (2) unobtainable supervised labels, (3) textual rather than raw sensory input, and / or (4) implausibly large memory (e.g. thousands of contextual words). These elements highlight the need to identify algorithms that, under these limitations, would suffice to account for both behavioral and brain responses. Focusing on the issue of speech processing, we here hypothesize that self-supervised algorithms trained on the raw waveform constitute a promising candidate. Specifically, we compare a recent self-supervised architecture, Wav2Vec 2.0, to the brain activity of 412 English, French, and Mandarin individuals recorded with functional Magnetic Resonance Imaging (fMRI), while they listened to ~1h of audio books. Our results are four-fold. First, we show that this algorithm learns brain-like representations with as little as 600 hours of unlabelled speech -- a quantity comparable to what infants can be exposed to during language acquisition. Second, its functional hierarchy aligns with the cortical hierarchy of speech processing. Third, different training regimes reveal a functional specialization akin to the cortex: Wav2Vec 2.0 learns sound-generic, speech-specific and language-specific representations similar to those of the prefrontal and temporal cortices. Fourth, we confirm the similarity of this specialization with the behavior of 386 additional participants. These elements, resulting from the largest neuroimaging benchmark to date, show how self-supervised learning can account for a rich organization of speech processing in the brain, and thus delineate a path to identify the laws of language acquisition which shape the human brain.

==> 10_intro.tex <==
\section{Introduction}
% General motivation
The performance of deep neural networks has taken off over the past decade. Algorithms trained on object classification, text translation, and speech recognition are starting to reach human-level performance \citep{xu2021self}. Furthermore, the \emph{representations} generated by these algorithms have repeatedly been shown to correlate with those of the brain \citep{kriegeskorte2015deep,yamins2016using,kietzmann2018deep,kell2019deep,cichy2019deep,toneva_interpreting_2019,millet2021inductive,caucheteux2022brains}, suggesting that these algorithms converge to brain-like computations. % temporal order

% Challenge
Such convergence, however, should not obscure the major differences that remain between these deep learning models and the brain. In particular, the above comparisons derive from models trained with 
(1) extraordinarily large amounts of data (40GB
for GPT-2 \citep{gpt2}, the equivalent of multiple lifetimes of reading), 
(2) supervised labels, which is rarely the case for humans (e.g. \citep{yamins2016using}),
(3) data in a textual rather than a raw sensory format, and/or
(4) considerable memory (e.g., language models typically have parallel access to thousands of context words to process text). These  differences highlight the pressing necessity to identify architectures and learning objectives which, subject to these four constraints, would be sufficient to account for both behavior and brain responses.

% Our approach
Here, we hypothesize that the latest self-supervised architectures trained on raw sensory data constitute promising candidates \citep{borgholt2022brief,bardes2021vicreg,Baevski2020wav2vec2A}. We focus on wav2vec 2.0 \citep{Baevski2020wav2vec2A}, an architecture that stacks convolutional and transformer layers to predict a quantization of the latent representations of speech waveforms. We train wav2vec 2.0 on 600\,h of \revised{effective} speech -- a quantity roughly comparable to what infants are exposed to during early language acquisition (speech only makes up a small fraction of infants' daily experience) \citep{dupoux2018cognitive,hart1992american,gilkerson2017mapping}.

We use standard encoding analyses  \citep{naselaris2011encoding,huth_natural_2016,yamins2016using,kell2018task} (Figure \ref{fig-methods})
%\citep{, nasarelis,yamins} 
to compare this model to the brains of 412 healthy volunteers (351 English speakers, 28 French speakers, and 33 Mandarin speakers) recorded with functional magnetic resonance imaging (fMRI) while they passively listened to approximately one hour of audio books in their native language \citep{nastase2020narratives,li2021petit} (8.5 hours of distinct audio materials in total).

To better understand the similarities between wav2vec 2.0 and the brain, we compare brain activity to each layer of this model, as well as to several variants, namely (1) a random (untrained) wav2vec 2.0 model, (2) a model trained on 600\,h of non-speech sounds, (3) a model trained on 600\,h of non-native speech  (for example, a model trained on English speech and mapped onto the brain responses to French-speaking participants), (4) a model trained on 600\,h of native speech  (for example, a model trained on English speech and mapped onto the brain responses to English participants), and (5) a model trained directly on speech-to-text (i.e., a supervised learning scheme) on the native language of the participants.

% Contribution
Our results provide four main contributions. First, self-supervised learning leads wav2vec 2.0 to learn latent representations of the speech waveform similar to those of the human brain. Second, the functional hierarchy of its transformer layers aligns with the cortical hierarchy of speech in the brain, and reveals the whole-brain organisation of speech processing with an unprecedented clarity. Third, the auditory-, speech-, and language-specific representations learned by the model converge to those of the human brain. Fourth, behavioral comparisons to 386 supplementary participants' results on a speech sound discrimination task confirm this common language specialization.
%develop language specific internal representations, similarly to to what's happening in humans. % Clarify the behavioral part here

% Our results provide three main contributions. First, self-supervised learning suffices wav2vec 2.0 to represent the speech wave form similarly to the human brain. Training wav2vec2.0 with a supervised objective decreases its similarity to the brain. Second, the functional hierarchy of its transformer aligns with the cortical hierarchy of speech in the brain. Third, the auditory, speech and language specifically learnt by the model converge to those of the human brain. These results strengthen the similarities observed between the behavior of this algorithms and those of human individuals.  % Clarify the behavioral part here

% Our results provide three main contributions. First, we show that self-supervised learning suffices for wav2vec 2.0 to reach human performance at sound discrimination, and to represent the speech wave form similarly to the human brain. Furthermore, the functional hierarchy of its transformer aligns with the cortical hierarchy of speech: the low-level representations of shallow layers map with the auditory cortex while the abstract semantic representations of the deeper layers aligns with associative brain regions. Finally, we find that the auditory, speech and language representations specifically learned by the model converge to those of the human brain. 


==> 20_methods.tex <==
\section{Methods}
\subsection{Models}

We train several variants of wav2vec 2.0 \citep{Baevski2020wav2vec2A} from scratch on different \revised{speech} datasets using two different learning objectives (a self-supervised and a supervised objective).


\subsubsection{Architecture}
Wav2vec 2.0 consists of three main modules. First, a feature encoder composed of seven blocks of temporal convolutions (output dimension 512) transforms the speech input $S$ (raw mono waveform at 16\,kHz) into a latent representation $z$ (output dimension of 512, frequency 49\,Hz, stride of 20\,ms between each frame, receptive field of 25\,ms). Second, a quantization module discretizes $z$ into $q$, a dictionary of discrete and latent representations of sounds. % (which are parameters of the model that can be learned) of the same dimension as $z$. %The quantizer will transform $z$ into the discrete representation that is the closest to it. 
Third, $z$ is input to a ``context network'' consisting of 12 transformer blocks (model dimension 768, inner dimension %--FFN-- 
3072, and 8 attention heads), which together yield a contextualized embedding $c$, of the same dimensionality of $q$. %We here train this architecture with two distinct objectives and three three types of audio datasets. 

\subsubsection{Learning objective}

\paragraph{Self-supervised learning.} In this training paradigm, the model optimizes two losses. The first loss is contrastive and requires the model to predict the quantized representation $q$ of some masked input using $c$, from a finite set of quantized representations drawn from the input sample. The second loss ensures that the quantized representations are diverse. See Section \ref{ap:loss_sup} and \citep{Baevski2020wav2vec2A} for details.

\paragraph{Supervised learning.} In this training paradigm, the quantization module is discarded and a linear layer mapping $c$ to phonemes is added at the end of the pipeline. The model is randomly initialized and all layers (including the feature encoder) are trained using a Connectionist Temporal Classification (CTC) \citep{graves2012connectionist} loss to perform phone recognition.
% 
For both training paradigms, we extract the activations of each layer from both the feature encoder (outputting $z$) and the context network (outputting $c$). We extract the representations of the convolutional and transformer blocks using an input window of 10\,s of raw waveform (stride = 5\,s).



\subsubsection{Training}
\label{sec-trainingimplem}
\paragraph{Datasets.} We successively train different wav2vec 2.0 models using each of four datasets: (i) the French and (ii) English CommonVoice corpora \citep{ardila2020common}, (iii) the MAGICDATA Mandarin Chinese Read Speech Corpus \citep{magicdata}, and (iv) a non-speech subset of the Audioset dataset \citep{gemmeke2017audio}, which contains recordings of various acoustic scenes.

\paragraph{Preprocessing.} All the audio datasets were randomly subsampled to have an approximate size of 600 hours, downsampled to 16\,kHz and converted to mono with the Sox software\footnote{\url{http://sox.sourceforge.net/}}. We randomly split the datasets into a training (80\%), a validation (10\%) and a test set (10\%). %\footnote{The exact subsets chosen can be delivered upon request} %\url{https://github.com/JAMJU/brain_and_models}}. 
The audio recordings we use from the Audioset dataset are filtered so that they do not contain speech or any sounds produced by humans, such as laughter or singing. %\footnote{The exact labels can be delivered upon request} %\url{https://github.com/JAMJU/brain_and_models}}. 
For the speech datasets, we also use their corresponding annotations (in the supervised settings). We phonemize these annotations using eSpeakNG\footnote{\url{https://github.com/espeak-ng/espeak-ng}}. The number of different phoneme symbols in these annotations is similar for French (32), English (39), and Mandarin Chinese (33).
% For the speech datasets, we also use their corresponding annotations (in the supervised settings). We phonemize these annotations using eSpeakNG\footnote{\url{https://github.com/espeak-ng/espeak-ng}}. Note that the number of different phoneme symbols in these annotations is similar for French (32), English (39), and Mandarin Chinese (33).

% \paragraph{Implementation.} We train all of our models using the fairseq implementation of wav2vec 2.0\footnote{\url{https://github.com/pytorch/fairseq/tree/main/examples/wav2vec}} using default hyperparameters.  We also analyze a model whose parameters were randomly initialised (``untrained'' model).

\paragraph{Implementation.} We train all of our models using the fairseq implementation of wav2vec 2.0\footnote{\url{ https://github.com/pytorch/fairseq/tree/main/examples/wav2vec}} using default hyperparameters.  We also analyze a model whose parameters were randomly initialised (``untrained'' model).

We use self-supervised learning to train four models: three on the speech datasets (French, English, and Mandarin) and one on the acoustic scenes dataset. In each case, the training was performed using the same configuration file (namely, the base configuration provided in the fairseq repository for pretraining wav2vec 2.0 on LibriSpeech \citep{panayotov2015librispeech}). We train the models for 400k updates and select the ones with the best validation loss.


We also use the supervised training paradigm to train three models, on the French, English, and Mandarin datasets, respectively. Each training was performed using the same configuration file, which was identical to the configuration provided in the fairseq repository for  fine-tuning wav2vec 2.0 on the 960 hour Voxpopuli corpus \citep{wang2021voxpopuli}, except that parameters were not frozen (\texttt{freeze\_finetune\_updates$=0$}) and learning was performed on all parameters of the models using the CTC loss (\texttt{feature\_grad\_mult$=0.1$}). We train the models for 400k updates and we use the ones with the best word error rate (WER) on the validation set. The French model obtains 13.9 WER, the English model 28.6 WER, and the Mandarin model 4.6 WER, on their respective test sets.




%\subsubsection{training datasets}
%\label{sec-trainingdata}


\subsection{Functional MRI}
\label{sec-fmridata}
We analyse a composite set of fMRI recordings aggregated from the \textit{Little Prince} \citep{li2021petit} and the \textit{Narratives} public datasets \citep{nastase2020narratives}.

% \paragraph{Narratives.} This is a public dataset\footnote{\url{https://openneuro.org/datasets/ds002345/versions/1.1.4}} consisting of the fMRI recordings of 345 native English-speaking participants listening to English narratives (4.6 hours of unique audio in total). Following \citep{nastase2020narratives}, we (1) focus on fifteen representative stories and ignore the narratives that have been modified by scrambling and (2) exclude eight participants because of noisy recordings. Overall, this selection results in a curated dataset of 303 participants listening to fifteen stories ranging from 3\,min to 56\,min, for a total of 4 hours of unique audio, 36018 words, and 4004 unique words. 

\paragraph{Narratives.} This dataset\footnote{\url{https://openneuro.org/datasets/ds002345}} contains the fMRI recordings of 345 native English-speaking participants listening to English narratives (4.6 hours of unique audio in total). \revised{The participants listened to different stories varying from 7 to 98\,min (mean\,=\,26\,min)}. Following \citep{nastase2020narratives}, we (1) focus on fifteen representative stories and ignore the narratives that have been modified by scrambling and (2) exclude eight participants because of noisy recordings. Overall, this selection results in a curated dataset of 303 participants listening to fifteen stories ranging from 3\,min to 56\,min, for a total of 4 hours of unique audio (36,018 words from a vocabulary of 4,004 unique words).

\paragraph{The Little Prince.} This dataset\footnote{\url{https://openneuro.org/datasets/ds003643/versions/1.0.4}} contains fMRI recordings of 48 English native speakers, 33 Mandarin native speakers, and 28 French native speakers listening to \textit{The Little Prince} in their respective native language.
%%% - N'EST-CE PAS VRAI POUR LES NARRATIVES AUSSI? PRAGMATIQUEMENT, IL FAUT PAS LE DIRE POUR L'UN ET NON PAS POUR L'AUTRE:
% All participants were right-handed, healthy volunteers, provided written informed consent prior to participation.  %%% 
The experiment itself was divided into nine runs of approximately 10\,min of passive listening. % of the story \textit{the Little Prince}. 
%
% We analyse the sound stimuli used during the fMRI collection in English, French, and Mandarin as input to our models.
For each language condition, the story was read by a single native speaker. %The corresponding audio files are included in the \emph{Little Prince} dataset. 
The English, Mandarin, and French audiobooks last 94, 90 and 97 minutes respectively. % For our experiments, we down-sample the recordings to 16\,kHz and convert them to mono with the Sox software \footnote{\url{http://sox.sourceforge.net/}}.


\paragraph{Preprocessing.}
For Narratives, we did not perform additional preprocessing: we use the public preprocessing of the dataset already projected on the surface space (``fsaverage6'') without spatial smoothing (labelled ``afni-nosmooth'' in the data repository). In contrast, the \textit{Little Prince} dataset is only provided in a volumetric space. Consequently, for each language condition separately, we subselected the cortical voxels by computing a brain mask using the average of all participants' fMRI data realigned onto a common template brain via Freesurfer \citep{freesurfer}. These voxels are then projected onto a brain surface using nilearn's {\texttt{vol\_to\_surf}} function with defaults parameters \citep{nilearn} and a `fsaverage6` template surface \citep{freesurfer}. 
%
For both \textit{Narratives} and \textit{The Little Prince}, fMRI signals are normalized across the time dimension to have a mean of 0 and a variance of 1, for each participant, surface voxel and session independently. 


\paragraph{Brain parcellation.} \label{parcellation}
For the purposes of certain analyses, %In Figure \ref{fig-prediction}.B,  \ref{fig-hierarchy}.C and \ref{fig-languages}.B, 
we group the fMRI voxels into regions of interest using the Destrieux Atlas \citep{destrieux_automatic_2010}. This parcellation results in 75 brain regions in each hemisphere. For simplicity, we label the regions as follows: A1 and A2 represents Heschl gyrus, which is the anatomical location of the primary and secondary auditory cortices, STG and STS are the superior temporal gyrus and sulcus, and IFG is the inferior frontal gyrus.



% \subsection{Neural Predictivity score ($R$)}
% % X = model's internal activations
% % W= linear_regression o hrf 
% \subsubsection{Temporal alignement}
% The sampling frequency of the model's activations (between 49 and 200\,Hz) is different from the sampling frequency of fMRI BOLD signals (0.5\,Hz). Furthermore, BOLD signals are known to be slow and to have delayed responses spanning over several seconds. To compare the activations of the models and the fMRI BOLD signals, we thus convolve the model activations  with a standard hemodynamic response function (HRF, $h$). The activations of the network $X \in \mathbb{R}^{d_{\hat{t}} \times d_x}$ are first normalized between $[0, 1]$ for each listening session. Then, we use nistats \citep{nilearn} \texttt{compute\_regressor} function with the `glover' model to temporally convolve ($h \in \mathbb{R}^{d_{\hat{t}}}$) and temporally down-sample ( using $g: \mathbb{R}^{d_{\hat{t}}} \rightarrow \mathbb{R}^{d_t}$) each artificial neuron $j$. See the formula of the operation in the appendix \ref{ap:preproc}.


% Note that both $h$ nor $g$ are fixed (i.e., not learnt). We used the default parameters as defined by nistats with the `glover' model in \texttt{compute\_regressor}. The transformed activations obtained are then normalised, per listening session, to have a mean of 0 and a variance of 1 for each dimension.


% \subsubsection{Model $\rightarrow$ Brain alignment: Neural Predictivity scores (R)}\label{np_score}

% We assess the similarity between the preprocessed model's activations $\hat{X} \in \mathbb{R}^{d_t\times d_x}$ and the BOLD response $Y\in \mathbb{R}^{d_t \times d_y}$ with a Neural Predictivity score (further denoted $R$ score). %, similar to  \citep{huth_natural_2016,yamins2016using,schrimpf_brain-score_2018}. 

% Specifically, we use a cross-validation evaluation setting within each subject (5 train-test splits). For each split $s$, we fit an $L_2$-regularized linear model $V \in \mathbb{R}^{d_x\times d_z}$ trained to predict the transformed BOLD time series from the model activations for each dimension independently. The formula of the optimisation objective is available in the appendix \ref{ap:ridge}. $W$ represents the complete encoding function from the model's internal activations to the BOLD predictions.

% Optimization is done using \texttt{RidgeCV} from scikit-learn \citep{pedregosa2011scikit}, with the penalization hyper-parameter $\lambda$ varying between 10 and $10^8$ (20 values scaled logarithmically) chosen independently for each dimension with a nested cross-validation over the training set.

% The performance of the ridge regression is summarized with a Pearson's correlation score between the predicted fMRI BOLD responses and the real ones on the test samples $\mathrm{test}_s$. We call this metric Neural Predictivity ($R$):

% \begin{equation}
%     R = \mathrm{Corr}(y_{\mathrm{test}_s}, W(x_{\mathrm{test}_s}))
% \end{equation}


\subsection{Brain score (R)}\label{np_score}
% X = model's internal activations
% W= linear_regression o hrf 

To quantify the similarity between the network's activations $X$ and the brain recordings $Y$, we use a standard linear encoding model \citep{huth_natural_2016,yamins2016using}. For each subject, we split the data into train and test sets using a five-fold cross-validation setting. For each train split, a linear mapping $W$ is fitted to predict the brain response $Y_{\mathrm{train}}$ given $X_{\mathrm{train}}$. $W$ combines a temporal alignment function with fixed weight, and a trained penalized linear regression.

\paragraph{Temporal alignment.} The sampling frequency of the model's activations (between 49 and 200\,Hz) differs from the sampling frequency of fMRI BOLD signals (0.5\,Hz). Furthermore, the BOLD signals have delayed responses spanning over several seconds. Thus, we first convolve the model activations  with a standard hemodynamic response function (HRF) using nistats \citep{nilearn} \texttt{compute\_regressor} function with the `glover' model and default parameters. This results in the convolved activations $X'_{\mathrm{train}}$ with the same sampling frequency as the fMRI $Y_{\mathrm{train}}$ (see \ref{ap:preproc}). 

% Precisely, the activations of the network $X \in \mathbb{R}^{d_{\hat{t}} \times d_x}$ are first normalized between $[0, 1]$ for each listening session. Then, we use nistats \citep{nilearn} \texttt{compute\_regressor} function with the `glover' model to temporally convolve.

\paragraph{Penalised linear regression.} Once temporally aligned, we fit an $\ell_2$-penalised linear regression that predicts the brain signals $Y_{\mathrm{train}}$ given the activations $X_{\mathrm{train}}$. We use the \texttt{RidgeCV} function from scikit-learn \citep{pedregosa2011scikit}, with the penalization hyperparameter $\lambda$ varying between 10 and $10^8$ (20 values scaled logarithmically) chosen independently for each dimension with a nested cross-validation over the training set (see \ref{ap:ridge}).

\paragraph{Evaluation.} We evaluate the linear mapping $W$ on the held out sets by measuring Pearson's correlation between predicted and actual brain responses:
%
% \begin{equation}
    $R = \mathrm{corr}\big(Y_{\mathrm{test}}, W \cdot X_{\mathrm{test}}\big)$. % \enspace .
% \end{equation}
%
Finally, we average the correlation scores across test splits to obtain the final ``brain score''. 
%
\label{circle_mean}
To report the average layer $k^*$ with the highest brain score for each voxel (Figure \ref{fig-hierarchy}), while being robust to regression-to-the-mean biases, we first find the best layer $k_s$ for each participant $s$ and each voxel independently and then compute a circular mean across the $N=412$ participants and the $K=19$ layers:
$
% \begin{equation*}
    % k^* = \mathrm{angle}\left(\frac{1}{N}\sum_{s=1}^N \cos(\frac{2\pi k_s}{K+1}) + i \sin(\frac{2\pi k_s}{K+1})\right)
    k^* = \mathrm{angle}\left(\frac{1}{N}\sum_{s=1}^N \exp\left(\frac{2i\pi k_s}{K+1}\right)\right)
% \end{equation*}
$

\paragraph{Statistics.}\label{stats}
We assess the reliability of brain scores with second-level analyses across participants thanks to a Wilcoxon signed-rank test across participants. Thus, the resulting p-values are not affected by fMRI auto-correlation within participants. We perform statistical correction for multiple comparisons with Benjamini–Hochberg False Discovery Rate (FDR) across voxels \citep{benjamini2010discovering}.%Figures only plot brain scores that are significant across participants after FDR correction ($p_{FDR}<0.05$). In the barplots, vertical lines and stars indicate significant gains ($\Delta R$) across participants: i.e., when the activations of a particular layer or a particular model better predict fMRI responses than another layer or model. One star corresponds to a p-value below $0.05$, two stars below $0.01$ and three stars below $0.001$.


% The performance of the ridge regression is summarized with a Pearson's correlation score between the predicted fMRI BOLD responses and the real ones on the test samples $\mathrm{test}_s$. We call this metric Neural Predictivity ($R$):

% \subsubsection{Temporal alignement}
% The sampling frequency of the model's activations (between 49 and 200\,Hz) is different from the sampling frequency of fMRI BOLD signals (0.5\,Hz). Furthermore, BOLD signals are known to be slow and to have delayed responses spanning over several seconds. To compare the activations of the models and the fMRI BOLD signals, we thus convolve the model activations  with a standard hemodynamic response function (HRF, $h$). The activations of the network $X \in \mathbb{R}^{d_{\hat{t}} \times d_x}$ are first normalized between $[0, 1]$ for each listening session. Then, we use nistats \citep{nilearn} \texttt{compute\_regressor} function with the `glover' model to temporally convolve ($h \in \mathbb{R}^{d_{\hat{t}}}$) and temporally down-sample ( using $g: \mathbb{R}^{d_{\hat{t}}} \rightarrow \mathbb{R}^{d_t}$) each artificial neuron $j$. See the formula of the operation in the appendix \ref{ap:preproc}.


% Note that both $h$ nor $g$ are fixed (i.e., not learnt). We used the default parameters as defined by nistats with the `glover' model in \texttt{compute\_regressor}. The transformed activations obtained are then normalised, per listening session, to have a mean of 0 and a variance of 1 for each dimension.


% \subsubsection{Model $\rightarrow$ Brain alignment: Neural Predictivity scores (R)}\label{np_score}

% We assess the similarity between the preprocessed model's activations $\hat{X} \in \mathbb{R}^{d_t\times d_x}$ and the BOLD response $Y\in \mathbb{R}^{d_t \times d_y}$ with a Neural Predictivity score (further denoted $R$ score). %, similar to  \citep{huth_natural_2016,yamins2016using,schrimpf_brain-score_2018}. 

% Specifically, we use a cross-validation evaluation setting within each subject (5 train-test splits). For each split $s$, we fit an $L_2$-regularized linear model $V \in \mathbb{R}^{d_x\times d_z}$ trained to predict the transformed BOLD time series from the model activations for each dimension independently. The formula of the optimisation objective is available in the appendix \ref{ap:ridge}. $W$ represents the complete encoding function from the model's internal activations to the BOLD predictions.

% Optimization is done using \texttt{RidgeCV} from scikit-learn \citep{pedregosa2011scikit}, with the penalization hyper-parameter $\lambda$ varying between 10 and $10^8$ (20 values scaled logarithmically) chosen independently for each dimension with a nested cross-validation over the training set.

% The performance of the ridge regression is summarized with a Pearson's correlation score between the predicted fMRI BOLD responses and the real ones on the test samples $\mathrm{test}_s$. We call this metric Neural Predictivity ($R$):

% \begin{equation}
%     R = \mathrm{Corr}(y_{\mathrm{test}_s}, W(x_{\mathrm{test}_s}))
% \end{equation}


% we then average the optimal layers $k^*$ across participants using a circle mean. We use a circle mean to avoid the regression to the mean effect. Precisely, we first project the possible values of $k$ ($k \in [0, 18]$) onto the trigonometric circle, deduce the corresponding angle $\theta_k$  ($\theta_k \in [0, 2\pi[$) and the angle $\theta_{k^*}$ that maximises the brain score for each (voxel, subject) pair. Then, we average the optimal $\theta_{k^*}$ across participants, and project back the averaged value $\bar \theta_{k^*}$ in the initial space. This results in an optimal average layer $\bar k^{*} \in [0, 18]$. 

\subsection{Behavioral experiment} \label{ABX}
\revised{To compare the phonetic representations of our models to those of humans, we compare the forced-choice discrimination judgements of online participants\footnote{\url{https://docs.cognitive-ml.fr/perceptimatic/}} to an analogous method applied to wav2vec 2.0 \citep{schatz2016abx}. 
Specifically, for each triplet of sound ``ABX'', participants judged whether the stimulus X was more similar to A or B. Analogously, we computed the Euclidean distance in the most discriminative layer of wav2vec 2.0 (here transformer layer 5) to determine whether X was closer to A or B. Additional data, analyses and model-human comparison can be found in \citep{millet2022self}.}
%
% To study the representation specific to each language,  we compare the way humans and models are able to discriminate native and non-native speech sounds. We use ``ABX'' tasks, which are discrimination tests during which participants have to listen to three speech sounds: A (e.g., /pop/), B (e.g., /pap/) and X (e.g., /pop/) \citep{schatz2016abx}. X is of the same category as A or B, and the participant has to decide which of A or B is the closest to X. Once the results are aggregated across participants of one given language group, the discrimination accuracy indicates whether they can differentiate the categories A and B belong to (in our example, whether they can differentiate the phone pair /o/-/a/). 
%
% For this, we use the Perceptimatic human benchmark\footnote{\url{https://docs.cognitive-ml.fr/perceptimatic/}} that contains the ABX results of French and English-speaking participants on speech stimuli from various languages.  
We focus on the French and English stimuli, which represent $\approx$ 6,000 ABX triplets (testing 508 English and 524 French phone pairs), with 386 participants in total (193 from each language group). 

In Figure \ref{fig-languages}-A, we report the ABX accuracy of English- and French-speaking participants in both their native and non-native language (either English or French). We first average results per phone pair, and then average over phone pairs to obtain the ABX discrimination accuracy. Similarly, in Figure \ref{fig-languages}-B, we compute the ABX accuracy of our wav2vec 2.0 models on the same evaluation sets as the participants, using the parameters described in \citep{millet2022self}. English and French models are evaluated on the same (`native') or different (`non-native') language stimuli as their training. The random and non-speech models are evaluated on both French and English speech stimuli.

% \subsection{Layer specificity}


%\begin{tabular}{lr}
%Acronym & Definition \\
%\midrule
% A1 / A2 & Primary / secondary auditory cortex \\
% STG / STS & Superior temporal gyrus / sulcus \\ 
% IFG & Inferior frontal gyrus  \\ 
%\bottomrule
%\end{tabular}
% \textcolor{red}{We also need to explain here how the ROI and plots are made.}


==> 30_results.tex <==
\section{Results}
\label{sec:results}

% \subsection{600\,h of self-supervised learning leads to the generation of brain-like representations}
\paragraph{Wav2vec 2.0 maps onto brain responses to speech.}
%To what extent does self-supervised learning over speech data suffices to learn representations similar to those of the human brain?
%To address this question, w
We estimate whether the activations of wav2vec 2.0 models linearly map onto the human brain activity of 412 individuals listening to audio books in the fMRI scanner.
%
%neural predictivity of  the NP score for the different training settings versions of the wav2vec 2.0 model to evaluate their ability to predict brain activity during a speech perception task for the three language groups in our two datasets.
%
%We call \textbf{native} the models that are trained on the native language of the participants of which they predict the brain activity of (e.g., English for English-speaking participants), and\textbf{non-native} the average of models that are trained on non-native languages of the participants of which they predict the brain activity of (e.g., French and Mandarin Chinese for English participants).
%
For this, we first independently train three models with 600\,h of French, English, or Mandarin, respectively, and 
compute the \revised{brain scores} ($R$) with the corresponding participants. Specifically, we (1) convolve the activations ($X$) of the model with a hemodynamic response function (HRF), (2) train a $\ell_2$-penalized linear regression on a training split to map them to brain activity $Y$, and (3) compute the Pearson correlation coefficient between (i) the true fMRI activity and (ii) the predicted activations on a test split.
% the model' activations convolved with a standard hemo-response dynamic response and a maximally aligned projection fit with a ridge regression. 
%We compare the resulting $R$ coefficients to those obtained with a randomly initialised model.
%
%We first assess the NP score obtained by native wav2vec 2.0 models, for all participants (Figure \ref{fig-prediction}.A). 
The models' activations significantly predict brain activity in nearly all cortical areas, reaching the highest $R$ scores in the primary and secondary auditory cortices (Figure \ref{fig-prediction}-A\,B). These scores are significantly higher than those obtained with a randomly initialised model ($p<10^{-50}$ on average across voxels), and this comparison is robust across language groups (all $p<10^{-5}$).
%
% We compare the native models' predictions to the results of an untrained (random) model (see Figure \ref{fig-prediction}.B for selected regions of interest, and Figure \ref{fig-prediction}.C for the whole brain).

%As previously reported\citep{millet2021inductive}, the activations of a random model significantly predict brain activity above chance, suggesting that deep convolutional neural networks present an important inductive bias.

%Self-supervised learning seems to be more biologically plausible as a way to model the learning process of humans. Indeed, self-supervised models do not use any external labels, but use only the audio input to develop relevant internal representations, and, in the case of wav2vec 2.0, they are trained to predict masked or future inputs, which we know human do \textcolor{red}{[CITE]} (\textcolor{red}{pb avec cette phrase je pense à revoir}). 

% However, most experiments that compared humans and models during a speech perception task have used supervised speech recognition systems \textcolor{red}{[CITE]}. Here, we study the impact of using either a supervised or a self-supervised goal to train our model.

% \subsection{Self-supervision leads to more brain-like representations than supervision}
\paragraph{Comparison of self-supervised to supervised models.}
Does self-supervision reach representations that are as brain-like as those obtained with supervised learning?
To address this issue, we trained wav2vec 2.0 with an alternative, supervised objective, namely, predicting phonetic annotations from the same 600 hours of \revised{effective} speech sounds. We then implemented the $R$ score analyses described above. The results show that self-supervised learning in fact leads to modestly but significantly better $R$ scores than supervised learning (Figure \ref{fig-prediction}-C): $\Delta R = 0.002, p<10^6$. %(grey bar) regarding developing internal representations that can linearly predict brain activity.

% This is important because, in opposition with during supervised training, our self-supervised wav2vec 2.0 models did not receive any other linguistic inputs than the speech audio recordings themselves. Without receiving informations about sound categories (phonemes) for example, self-supervised wav2vec 2.0 managed to develop internal representations that seem to reproduce speech processing in the brain. 

%In particular, the representational space developed during training seem to follow the main sound categories developed by phoneticians. We show this by applying a t-SNE analysis on the output of the model's  (see Figure \textcolor{red}{XXX}). 

% \subsection{Self-supervision leads to a functional hierarchy similar to the brain}
\paragraph{The hierarchy of wav2vec 2.0 maps onto the hierarchy of the cortex.
% Similar functional hierarchies.
}
To compare the speech hierarchy in the brain with the functional hierarchy learned by wav2vec 2.0, we evaluate the $R$ score of each layer of the model (Figure \ref{fig-hierarchy}). % summarizes the most predictive layer (on average across participants). Because this analysis may be subject to a regression-to-the-mean artefact, whereby noise biases the best layer to the middle one, we also report the layer-wise scores average across voxels (Figure \ref{fig-hierarchy}.B) as well as the proportion of voxels, which, after averaging across participants, are best predicted by a given layer (Figure \ref{fig-hierarchy}.C).
%
First, we observe that convolutional layers are less predictive than transformer layers. Second, within the transformers, the hierarchy of representations aligns with the expected cortical hierarchy \citep{hickok2007cortical}: while low-level areas (A1, A2) are best predicted by the first transformer layers, higher level areas (IFG, STS) are best predicted by deeper layers. Remarkably, this hierarchy extends to supplementary motor and motor areas in both hemispheres (Figure \ref{fig-hierarchy}-A). 
%When looking at the best predicting layer for each voxel in the brain (see Figure \ref{fig-hierarchy}.A), it appears that the speech processing hierarchies are similar between the model and what we know of the way our brain deals with speech.
% \maydelete{Some voxels around the auditory cortices seem to be tuned to the highest layers of wav2vec 2.0. Additional research focusing on a higher resolution of this region remains necessary to disentangle the role that feedback may play to explain this unexpected phenomenon.}

% \subsection{Evidence for a brain-like specialisation of acoustic, speech and language representations}
\paragraph{Language specificity in phone discrimination tasks.}%Language specialization: 
% Similar performance on a speech discrimination task.
% wav2vec 2.0 and participants

% }
The acoustic features underlying speech (fricatives, vowels, and so on) may also characterize non-speech sounds (the sound of tree leaves in the wind, of a stone falling, and so on). Does the model show commonalities merely with general auditory processing in the brain, or does it capture speech-specific processing? If so, does it show commonalities with brain representations that are specific to the native language of the participants, or merely to general speech processing?
% As self-supervised learning can be applied to any kind of audio data, it offers us the opportunity to study how data influences the model's ability to map onto brain responses to speech. 
%
We first evaluate the specialization of humans' perception to their native language using an ABX behavioral task (Section \ref{ABX}). Specifically, we compare 386 French and English participants on their ability to distinguish native and non-native phones. 
%We look at the ABX accuracy (see ) obtained by French- and English-speaking participants on English and French stimuli, see Figure \ref{fig-languages}.A. 
%We show that, as expected, 
As expected \citep{bohn2017cross,kuhl2005early}, participants were better at discriminating native sounds than non-native ones (across phone pairs: $p<10^{-18}$, Figure \ref{fig-languages}-A). 
Second, applying the same test to our self-supervised French and English models shows that, like humans, %models' discriminability was highest for native speech sounds (Figure \ref{fig-languages}.B): 
models best discriminate sounds from their `native' language (i.e., the French model better distinguishes French stimuli than English ones, across phone pairs, and vice versa: $p<0.05$). %obtain a better ABX accuracy than non-native models (\emph{e.g.} French model tested on English stimuli). 
\revised{
%{\color{red} [ABX]} Several qualitative and quantitative similarities have been recently observed between the behavior of wav2vec 2.0 and humans \citep{millet_self-supervised_2022, adolfi_successes_2022}. 
Interestingly, the ABX accuracy of the model is significantly higher than participants’. This quantitative difference may be partially explained by the fact that participants – and online participants in particular – undergo fluctuating attention, and adopt strategies which can negatively impact performance \citep{humphreys_acquisition_1939}. 
% More systematic comparison may, however, be necessary to identify and understand the core differences that remain between humans and this model \citep{adolfi_successes_2022}.
}
Finally, as expected, the random and acoustic models %on the same discrimination task: our model trained on non-speech sounds obtains 
obtain the worst ABX accuracy. % (\textcolor{red}{p-value}), and the random model is even worse (\textcolor{red}{p-value}). 
%
%
Overall, These results confirm that 600\,h of self-supervised learning on \revised{effective} speech suffices for wav2vec 2.0 to learn language-specific representations (Figure \ref{fig-languages}-B).

\paragraph{Wav2vec 2.0 and the brain learn language specific representations.}%Language specialization: similar neural representations.

Next, we compare the \revised{brain scores} of random, non-speech, non-native and native models (Figure \ref{fig-languages}-C\,D). 
% (1) a random model, (2) a model trained on non-speech sounds, (3) a model trained on speech in a language different from the participants (here referred to as "non-native models", \emph{e.g.} models trained on French and Mandarin and tested on their ability to predict brain responses to English speech), and (4) native models (Figure \ref{fig-languages}).
%
%If we now focus on the $R$ scores of these different models, o
First, our results show that the non-speech model attains higher $R$ scores than the random model (on average across voxels, $\Delta R = 0.006$, $p=10^{-31}$) confirming the importance of learning to generate brain-like representations. Second, non-native models attain higher $R$ scores than the non-speech model ($\Delta R=0.002, p=10^{-9}$), confirming that wav2vec 2.0 learns speech-specific representations of sounds when trained on speech. Finally, the native model attains higher $R$ scores than non-native models ($\Delta R=0.002, p=10^{-15}$). %This results reveals where the brain represents language-specific features. %, and that this specialization of our mental world can -- at least partially -- be captured by a self-supervised model like wav2vec 2.0.
%
% already leads to a great improvement in NP scores compared to a random model (ii) training on speech (whatever the language) is, however, always better in terms of NP scores (iii) the best NP scores are always obtained by the native models: training on the native language of the participants leads to the best brain-model similarity during a speech perception task.
%
%
%%% PREVIOUS VERSION %%%
% The specialization for native sounds shared between models and the brain appears to be mainly localized around the superior temporal sulcus and the middle temporal gyrus (Figure \ref{fig-languages}D), whereas higher-level regions like IFG and the angular gyrus only show more general specializations (i.e., speech rather than native-language sounds). 




%, non-speech audio representations can be detected in a vastly distributed set of cortical regions, whereas language-specific regions can be primarily recovered from the brain areas typically associated with speech processing, namely the infero-frontal, middle and superior temporal and angular cortices.% \textcolor{red}{say something about locality of the improvements}


%\textcolor{red}{Point out that 1) self-supervised training more biologically plausible 2) self-supervised more brain like that supervised 3) No need of explicit linguistic categories (maureen figure) 4) Loss of wav2vec can predict brain activity on its own}




==> 40_discussion.tex <==
\section{Discussion}
\label{sec-discussion}
% - Neuro: 
%     - hierarchie layer
%     - specificte de langue
% - Network: specificte de langues
% => self supervised, loss.

% 1. Question
Human infants acquire language with little to no supervision: A few hundred hours of speech suffices for their young brain to learn to discretize phonemes, segment morphemes, and assemble words in the language(s) of their social group \citep{dupoux2018cognitive,gilkerson2017mapping}. %The computational principles that allow this unique ability remains, to date, unknown.
% Here, we test whether self-supervised learning on a limited amount of speech suffices to yield a model functionally equivalent to speech perception in the human brain. 
\revised{However, the learning principle that allows this unique feat remains, to date, unknown.

Here, we test whether self-supervised learning applied to a limited amount of speech effectively accounts for the organization of speech processing in the human brain as measured with fMRI. For this, }we train several variants of wav2vec 2.0 \citep{Baevski2020wav2vec2A} with three curated datasets of French, English, and Mandarin, and compare their activations to those of a large group of French, English, and Mandarin speakers recorded with fMRI while passively listening to audio stories.
% 2. Main results
Our results show that this self-supervised model learns (i) representations that linearly map onto a remarkably distributed set of cortical regions (Figure \ref{fig-prediction}), (ii) a \revised{computational} hierarchy that aligns with the cortical hierarchy (Figure \ref{fig-hierarchy}), and (iii) features specific to the language of the participants (Figure~\ref{fig-languages}). %Finally, the comparison between different training regimes shows that this model learns both representations specific to each of the languages presently studied, namely French, English or Mandarin.

% DO WE HAVE ADDITIONAL BEHVIORAL RESULTS TO DISCUSS? e.g. 
% - ABX test on native versus non native
% - BLIMP/BiGBench on wav2vec (or speech equivalent done by Dupoux's team

% 3. Related work
\paragraph{Towards a biologically-plausible learning principle.} These results extend recent findings on the similarities between the brain and a variety of deep learning models trained with biologically-implausible objectives and data.
% 3.1. supervised audio models
First, fMRI \citep{kell2018task,millet2021inductive,thompson2021training}, electroencephalography \citep{huang2018connecting}, and multi- or single-unit responses to sounds  \citep{koumura2019cascaded,begus2022encoding} have been shown to be linearly predicted by the activations of deep convolutional networks trained on \emph{supervised} auditory tasks. For example, \citep{millet2021inductive} showed that a supervised \revised{speech-to-text} model better accounted for brain responses to speech in 102 individuals when it was trained on speech recognition rather than auditory scene classification. Similarly, \citep{kell2018task} showed that eight participants listening to brief speech and non-speech sounds demonstrated fMRI responses in the temporal lobe that aligned with those of a deep convolutional neural network trained on a binary auditory classification task. %A similar approach, although unsuccessful, was undertaken by \citep{thompson2021training}, who recorded six participants on a triphone recognition task with a 7-Tesla fMRI to compared to a supervised deep convolutional neural network. 
% our contribution
Our results, based on up to 50 times more fMRI recordings of the entire cortex show that such representational similarities hold with a self-supervised objective \citep{lerner_topographic_2011, berezutskaya2017neural,caucheteux_model-based_2021,caucheteux_long-range_2021}.
% 
% 3.2 unsupervised text models
Second, a growing series of MEG \citep{toneva_interpreting_2019,caucheteux2022brains}, fMRI \citep{mitchell2008predicting,qian2016bridging,pereira2018toward,schwartz2019inducing,antonello2021low,jain2018incorporating} and electro-physiology studies \citep{schrimpf2021neural,goldstein2022shared} showed that text-based language models trained on very large corpora generate brain-like representations too. 
%In particular, \citep{caucheteux2022brains} showed that the better language models were at predicting words from context, the more their representations mapped onto brain activity. Similarly, \citep{caucheteux_2021} showed that the more participants understand stories, as assessed with a questionnaire, the more their brain activity aligns with GPT-2 \citep{gpt2}. 
% Our contribution
While these results suggest elements of convergence between language models and the brain \citep{caucheteux2022brains}, they also remain biologically implausible: not only are these algorithms pre-equipped with abstract linguistic units such as characters and words,  but they are trained on corpora that no one would ever be able to read in their lifetime. In contrast, wav2vec 2.0 is here trained with a reasonable amount of raw speech waveforms \citep{hart1992american,gilkerson2017mapping,dupoux2018cognitive}. \revised{The functional similarity between wav2vec 2.0 and the brain thus opens the way to clarify how humans learn to process speech.}
% The self-supervised learning of wav2vec 2.0 is considerably more realistic than the classic supervised models

% 4. Neuroscientific findings
\paragraph{The emergence of a brain-like hierarchy of speech processing.}
The present study reveals the hierarchical organization of speech processing with remarkable clarity.
First, the functional hierarchy learnt by wav2vec 2.0 is aligned with the anatomy: \emph{e.g.} the superior temporal sulcus and the temporal pole are known to project to the ventral and dorsal part of the inferofrontal gyrus, respectively \citep{petkov_different_2015}.
Second, the identification of functional gradients within the prefrontal cortex, and down to the motor areas typically associated with larynx and mouth control \citep{dichter2018control} reinforces the relevance of motor processes to speech perception \citep{kellis2010decoding,mugler2014direct,shamma2021learning}. %% ???
Finally, the existence of multiple levels of representations around the inferofrontal cortex
is consistent with the idea that Broca's area may be responsible for merging linguistic units 
%% can't have may be .. may be, need to reformulate
%may be essential to understanding how Broca's area may be responsible for merging linguistic units 
\citep{chomsky2000linguistics,friederici1999neurobiology,hagoort2005broca,poeppel2012towards}. It should be noted, however, that our results aggregate a large cohort of individuals which could mask a more modular organization at the individual level.

\revised{
\paragraph{Interpreting the neural representations of speech. } 
Interpreting neural representations is a notoriously difficult challenge to both AI and neuroscience. Here, we first investigate language specificity and show that the neural representations specific to the native models are primarily represented in the superior temporal sulcus and middle temporal gyrus  (Figure \ref{fig-languages}D): areas known to represent phonetic features \citep{mesgarani_phonetic_2014}. % Interestingly, the specialization for native sounds shared between models and the brain appears to be mainly localized around the superior temporal sulcus and the middle temporal gyrus (Figure \ref{fig-languages}-D). 
%
% This suggests that these regions are uniquely sensitive to the fine auditory structures specific to each language, and that higher level regions, such as prefrontal and parietal cortices, may not retrieve such fine-grained features. {\color{red}Although preliminary, this result could support the classical view of modular processing in the cortex (e.g. \citep{fodor_modularity_1983}), whereby higher level regions (PFC) may be input with the \emph{result} of sensory hierarchy but would remain blind to its many intermediary features.}}
%
% \maydelete{While high-level areas are best predicted by the upper-middle layers, these layers actually correlate with several regions across cortex. Such observation is consistent with the recent results of \citep{vaidya2022self} and will necessitate carefully-controlled words and speech sounds to be tested explicitly}.
%
% \maydelete{Second, this region appears to capture the representations specifically learnt by the native models %Together, these results thus strengthen the show where phonetic representations are shaped by our experience \citep{liberman_discrimination_1961, werker_cross-language_1984, kondaurova_relationship_2009}. 
However, these effect are relatively modest (Figure \ref{fig-languages}): the random model and the non-speech model reach, in STS and STG, 67\% and 87\% of the \revised{brain scores} obtained by the ``native'' model, respectively. While this high baseline initially surprised us, this phenomenon could be explained by the fact that the auditory cortex is continuously bombarded by -- and should thus be tuned to -- non-speech input. %These elements thus highlight the importance of using large amounts of neuroimaging data to effectively compare minimally different models of speech in natural settings.
}
\revised{Second, our probing analyses show that the models trained with self-supervised learning learn relevant acoustic and linguistic representations (Supplementary Figure \ref{fig-probe}). This result, consistent with \citet{vaidya2022self} and \citet{stephenson2019untangling}, suggests that the difference of \revised{brain scores} observed between the random, non-native and native models (Figure \ref{fig-languages}) may be partly driven by the corresponding spectro-temporal, phonetic, word and sentence-level representations, respectively. These elements of interpretation remain, however, scarce, and a systematic interpretation of the representations shared between wav2vec 2.0 and the brain remains necessary.  %These results are consistent with the recent in-depth analyses of \citep{vaidya2022self} and will necessitate carefully-controlled words and speech sounds to be tested explicitly.
}

% \revised{\paragraph{Interpretability of wav2vec2.0. features.} Interpreting the representations of deep learning models is notoriously difficult, and the topic of dedicated studies. For example, \citep{pasad2021layer} explored the encoding of local acoustic features, phone identity, word identity and word meaning across layers. Similarly, \citep{millet-etal-2021-predicting} compared representations to human behavioural data to assess whether they better captured listeners' perception of higher-level phonemic properties or of lower-level subphonemic properties of speech stimuli. Finally, \citep{vaidya2022self} recent study explores filter banks, spectrograms, phonemes and words across layers. Here, we complement these analyses by showing that self-supervised learning allows wav2vec 2.0 to learn represents, along its hierarchy the representations of MEL spectrograms, phonetic categories and word embeddings (Figure \ref{fig-probe}).}

% \revised{Critically, only the highest-level features, namely phonetic- and word- and sentence-level features appeared to be specific to (1) speech and (2) to the language with which it was trained (Figure \ref{fig-probe}). Interestingly, the word and sentence-level features are encoded deeper in the supervised network (best layer=18 in Table \ref{tab:probe}) compared to the unsupervised network (best layer=14), which suggests that self-supervised learning generates a reservoir representations in its middle layers, reservoir which may partly overlap with the labels used in supervised learning. Together with our ABX tests, and layer-wise tuning of each voxel (Figure \ref{fig-hierarchy}), these elements suggest that the representations of speech shaped by our experience are learnt and instantiated in the superior temporal gyrus and sulcus. These elements, \revised{consistent with previous electrophysiological studies \citep{mesgarani_phonetic_2014}}, thus provide a coherent spectrum of evidence for the location of acquired speech representations in the brain.}

\revised{ 
\paragraph{Scope of the study.} It is important to stress that the scope of the present study could be broadened in several ways. First, our study focuses on adult speakers, whose cultural and educational background is not representative of the population \citep{henrich_weirdest_2010}. Second, we focus on the passive listening of three languages. Third, we focus on one self-supervised learning architecture \citep{Baevski2020wav2vec2A}, and its functional alignment with fMRI, whose temporal resolution is notoriously limited. Generalizing the present approach to more languages \citep{malik-moraleda_investigation_2022}, a larger spectrum of children and adult participants recorded with a variety of electrophysiological and neuroimaging devices will thus be essential to confirm, precise, and/or mitigate the present findings.}


\revised{ 
\paragraph{The remaining gap between brain and speech models.} 
%Our study shows that a self-supervised model, trained on a remarkably small amount of unlabelled data, effectively accounts for cortical responses to speech. 
% Our results certainly do not imply that wav2vec 2.0 has learned \emph{all} of the speech representations of the brain. Indeed, s
Several major gaps can be evidenced between wav2vec 2.0 and the brain. First, the transformer layers are not temporally constrained: each layer can access all elements within the contextual window. This differs from the necessarily recurrent nature of processing in the brain. Second, wav2vec 2.0 behaves differently to humans in specific tasks. In particular, it is overly-sensitive to band-pass filtering, non-robustly exploit fine temporal structures \citep{weerts2021psychometrics} and fails to display the expected categorical responses \citep{millet-etal-2021-predicting}. Third, recent studies show that wav2vec 2.0 encodes significantly less semantic information than text-based models \citep{pasad2021layer,vaidya2022self}. While our analyses suggest that learning allows wav2vec 2.0 to capture some lexical features in its deep layers (Figure \ref{fig-probe}, Table \ref{tab:probe}), it remains unclear whether these layers also capture complex syntactic structures, such as recursive syntactic trees \citep{lakretz_can_2021, caucheteux_disentangling_2021}. We speculate that these limitations may be due to the time scales of wav2vec 2.0 which, unlike humans, learns very short-term representations of speech.
In any case, these differences likely explain why the \revised{brain scores} of wav2vec 2.0 remain substantially lower than our noise-ceiling (19\% on average, and up to 74\% in Heschl’s gyrus and sulcus, Table \ref{tab:np_noiseceil}, Figure \ref{fig-noiseceil}). 

%Together with epistemological accounts \citep{guest_how_2021} and concurrent results \citep{vaidya2022self}, our results highlight the remaining gap between current self-supervised models and the human brain.
}

% 5. Limits and Impact
% \revised{\paragraph{Limitations} Our study shows that a self-supervised model, trained on a remarkably small amount of unlabelled data, effectively accounts for cortical responses to speech. This learning scheme is considerably more realistic than the classic supervised models, thus promises to help understand how the human brain learns and organizes speech processing.
% However, these results do not imply that wav2vec 2.0 has learned all of the speech representations used by the brain. Indeed, several major gaps remain between self-supervised speech models like wav2vec 2.0 and the brain.}
% %Still, several major gaps remain between self-supervised speech models like wav2vec 2.0 and the brain. 
% First, its transformer layers are not temporally constrained: each layer can access all elements within the contextual window. This differs from the necessarily recurrent nature of processing in the brain. Second, wav2vec 2.0 shows differences with humans in recent behavioral studies: it shows a heightened sensitivity to band-pass filtering and an under-reliance on fine temporal structures \citep{weerts2021psychometrics}. It also fails to predict categorical effects on perception \citep{millet-etal-2021-predicting}. \revised{Third, recent studies show that wav2vec 2.0 encodes significantly less semantic information than text-based models \citep{pasad2021layer,vaidya2022self}. Our analyses suggest that learning allows wav2vec 2.0 to capture some lexical features in its deep layers (Figure \ref{fig-probe}, Table \ref{tab:probe}). However, whether these layers also capture complex syntactic structures, such as recursive syntactic trees, remains an open question \citep{lakretz_can_2021}.}
% %Third, recent studies show that wav2vec 2.0 encodes significantly less semantic information than text-based models \citep{pasad2021layer}.
% %
% \revised{Finally, unlike humans, wav2vec 2.0, learns very short-term representations of speech. These differences likely explain why the neural predictivity scores of wav2vec 2.0 remain substantially lower than our noise-ceiling (19\% on average, and up to 74\% in Heschl’s gyrus and sulcus, Table \ref{tab:np_noiseceil}, Figure \ref{fig-noiseceil}). Together with epistemological accounts \citep{guest_how_2021} and concurrent results \citep{vaidya2022self}, our results highlight the remaining gap between current self-supervised models and the human brain.}
%
% OLD VERSION: These limitations may be due to the time scales of wav2vec 2.0 which, unlike humans, learns very short-term representations of speech. Overall, given that the human brain remains the best known system for speech processing, our results highlight the importance of systematically evaluating self-supervised models on their convergence to human-like speech representations.

Overall, the complexity of the human brain is often thought to be incompatible with a simple theory: ``Even if there were enough data available about the contents of each brain area, there probably would not be a ready set of equations to describe them, their relationships, and the ways they change over time''  \citep{gallant2013reading}. By showing how the equations of self-supervised learning give rise to brain-like processes, this work contributes to challenge this view. 

==> XX_checklist.tex <==

%%% BEGIN INSTRUCTIONS %%%

%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section \ref{sec:results}}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec-discussion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have, and since we use results of human experiments that were previously made, and that respect these review guidelines, we conform to them.}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{No theoretical results}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{No theoretical results}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code will be provided upon request. Otherwise for the rest, see Section \ref{sec-fmridata} and \ref{sec-trainingimplem}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{sec-trainingimplem}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{This is the case for all our figures, see Figure \ref{fig-prediction}, \ref{fig-hierarchy} and \ref{fig-languages}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{The models we train are not new: the original papers already give that type of information.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section \ref{sec-fmridata}, \ref{sec-trainingimplem}, and \ref{ABX}.}
  \item Did you mention the license of the assets?
    \answerNo{They are all under CC0 for the English and French training audio data, the Perceptimatic Benchmark, The Little Prince dataset and the Narratives dataset. Magic data is under CC BY-NC-ND 4.0, Audioset is under CC BY 4.0 for the audio recordings, and CC BY-SA 4.0 for the ontology, Narratives' preprocessing code is under GNU GENERAL PUBLIC LICENSE  and fairseq code is under MIT License.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{The code will be given upon request}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See Section \ref{sec-fmridata} and \ref{ABX}. More details on the way they gave their consent can be seen in the original papers/websites that provided the experimental results.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{The data were anonymized before we used them. }
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not conduct the experiments ourselves}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We did not conduct the experiments ourselves}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We did not conduct the experiments ourselves}
\end{enumerate}


\end{enumerate}

==> figures.tex <==

% \begin{SCfigure}
%   \centering
%   \includegraphics[width=0.6\textwidth]{figures/Figure1.png}
%   \caption{\textbf{Methods to compare speech representations deep networks and the brain.}}
% \label{fig-methods}
% \end{SCfigure}


\begin{figure}
  \centering
%   \includegraphics[width=0.94\textwidth]{figures/Figure1.png}
  \includegraphics[width=\textwidth]{figures/Figure1.png}
 % \includegraphics[\textwidth,trim={0 0.5cm 0 0},clip]{figures/Figure1.png}
  \caption{\textbf{Comparing speech representations in brains and deep neural networks.}
   \textbf{A.} We analyze the brain activity of 412 participants recorded with functional Magnetic Resonance Imaging (fMRI) while they passively listened to audio books in their native language (French, English or Mandarin). 
   %
   \textbf{B.} After training wav2vec 2.0 \citep{Baevski2020wav2vec2A} with self-supervised learning ($L$) over 600\,h of unlabelled, effective speech, %(either acoustic scenes, French, English or Mandarin speech), and 
   we extract its activations in response to the audio books that were presented to the participants.
    We assess the similarity between the activations of the model $X$ and brain activity $Y$ with a standard encoding model $W$ \citep{nastase2020narratives} evaluated with a cross-validated Pearson correlation $R$. %Precisely, a linear regression $W$ is fitted to predict the brain response $Y$ given $X$, the network activations convolved with a hemo-dynamic response function (HRF). 
    %
    \textbf{C.} Example\revised{s} of the true BOLD response (black) and the predicted BOLD response (red) estimated from a linear projection of the model's activations in \revised{three voxels randomly selected from the $10^{th}$ percentile of best voxels identified by the noise ceiling analysis for the first 200\,s of a representative story in the test set}.
    %To evaluate the resulting alignment, we compute the neural predictivity score, i.e. Pearson's correlation between predicted and actual brain activity on held out data (further denoted $R$). For instance, \textbf{C.} displays the actual (black) and predicted (red) activity (BOLD signal) for one particular voxel and subject.}
   % This score summarises the similarity between the speech representations in one deep network and the brain.
   }
\label{fig-methods}
\end{figure}


\begin{figure}[ht]
  \centering
  \includegraphics[width=\textwidth]{figures/Figure2.png}
  \caption{\textbf{Self-supervised learning suffices for wav2vec 2.0 to generate brain-like representations of speech.} 
  %\caption{\textbf{A self-supervised model accurately predicts brain activity.} 
  % We compute the brain scores of wav2vec 2.0. trained with either a self-supervised or supervised objective on 600 hours of audio. 
  %
  \textbf{A.} %Similarity between (i) the brain recordings of the 412 subjects listening to audio in their native language and (ii) the concatenated activations of wav2vec2, trained with a self-supervised objective on 600 hours of audio of the same language. 
  \revised{Brain score} ($R$) assessed for each subject and voxel independently, and here averaged across subjects for clarity. Only scores significantly above chance level, as assessed using a two-sided Wilcoxon test across subjects after correction for multiple comparison are color-coded ($p<10^{-10}$).
  %
  \textbf{B.} $R$ scores for the same wav2vec2 model, averaged across subjects and voxels in four brain areas typically involved during speech processing (the primary and secondary auditory cortices, the superior temporal gyrus, the superior temporal sulcus, and the infero-frontal gyrus). In grey, the brain score obtained with a randomly initialized wav2vec 2.0 architecture. Error bars are the standard errors of the mean (SEM) across subjects. The stars indicate a significant difference between the random and trained model (all $p<10^{-4}$).
  %
  \textbf{C.} $R$ scores of wav2vec 2.0 without training (top), trained with a supervised (middle) and self-supervised learning rule (bottom), on the same 600\,hours of effective speech. Scores are averaged across subjects and voxels and error bars are SEM across subjects.
  } 
\label{fig-prediction}
\end{figure}

\begin{figure} %[ht]
  \centering
  \includegraphics[width=0.9\textwidth]{figures/Figure3.pdf}
  \caption{\textbf{The functional hierarchy of wav2vec 2.0 maps onto the speech hierarchy in the brain.} 
  \textbf{A.} We compute the $R$ score for each layer of wav2vec 2.0 separately and estimate, for each voxel, the layer with highest brain score on average across subjects. Only the voxels with significant brain scores are displayed ($p<10^{-18}$). While the first transformer layers (blue) map onto the low-level auditory cortices (A1 and A2), the deeper layers (orange and red) map onto brain regions associated with higher-level processes (e.g. STS and IFG).
  %
  \textbf{B.} Layer-wise $R$ scores averaged across all voxels. Error bars are SEM across subjects. 
  %
  \textbf{C.} Proportion of voxels with most predictive layer (x-axis) in four regions typically involved in speech processing. While most voxels in the primary cortex are best predicted by the first layers of the transformer, higher-level brain areas are best predicted by deeper layers. %\color{red}{(3) clean diagram in A. (4) I'm wondering whether we shouldn't add the brain for average across subjects first}
  }
\label{fig-hierarchy}
\end{figure}

% \vspace[-1]

\begin{figure}[ht]
  \centering
  \includegraphics[width=\textwidth]{figures/Figure4.png}
\caption{\textbf{The specialization of wav2vec 2.0's representations follows and clarifies the acoustic, speech, and language regions in the brain.} \textbf{A.} We first evaluate humans' language specificity by quantifying their ability to perceive phonemes of their native or non-native languages (Section \ref{ABX}) in a ABX matching-to-sample task \citep{schatz2016abx} (higher is better). As expected, humans are better at matching phonemes of their native language. \textbf{B.} Then, we train four wav2vec 2.0 models with self-supervised learning on four datasets -- non-speech acoustic scenes, English, and French, and compute their ABX accuracy on the same speech datasets as humans. The `random' model is wav2vec 2.0 without any training. %We also report the ABX of one untrained wav2vec 2.0 model (`random').  %The speech models are tested on both the same (`native’) and different (`non-native’) languages as their training set. The non-speech and random models are evaluated on English speech. 
\textbf{C.} \revised{Brain score} ($R$) of each model (with an added model trained on Mandarin), averaged across voxels, in four regions of the brain (Section \ref{parcellation}). \textbf{D.} Acoustic, speech and language specificity for each voxel. For instance, one voxel is considered specific to the `native’ model if its native $R$ score is higher than its `non-native’ $R$ score ($p<.05$). Only the voxels with significant $R$ scores for the untrained model are displayed ($p<10^{-18}$). Error bars are the SEM across phone pairs in A and B, and across subjects in C. The stars indicates a significant difference between two conditions (Section \ref{stats}).
}
\label{fig-languages}
\end{figure}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\textwidth]{figures/Figure4.png}
%   \caption{\textbf{The specialization of wav2vec 2.0's representations follows and clarifies the acoustic, speech, and language regions in the brain.} 
%   %
%   %To quantify the functional specialisation of audio, speech and language representations, 
%   To study acoustic, speech and language specificity, we train from scratch four wav2vec 2.0 models with self-supervised learning on four datasets -- acoustic scenes, English, French and Mandarin.
%   %-- and compare them with one another as well as with an untrained wav2vec 2.0 model. , and compute their Neural Predictivity scores ($R$) in different parts of the brain.
%   \textbf{A)} We first evaluate the models using a behavioural metric, the `ABX' accuracy \citep{schatz_evaluating_2013}, which measures the ability to discriminate phones (Section XXXX), on a speech dataset of the same (`native') language training language
%   % ABX accuracy of the wav2vec 2.0 models when evaluated on a dataset of the same (`native') or different language (`non-native') as their training set. The non-speech and random models (untrained wav2vec 2.0) are evaluated on English speech. Error bars are standard error of the mean across phone pairs. \textbf{B)} ABX accuracy of English and French participants on the same evaluation sets. \textbf{C)} Neural Predictivty score ($R$) of the models averaged across the voxels of four brain regions typically associated with speech processing. The stars indicate a significant difference between the average brain scores of two models. \textbf{D)} Specificity of each voxel for each level of representations -- acoustic, speech and language. For instance, a voxel is marked `pink' if the $R$ score of the non-native models is significantly higher than the $R$ score of the non-speech model ($p<.05$). Only the voxels with significant $R$ scores for the untrained model are displayed ($p<10^{-18}$).
%   }
%     \label{fig-languages}
% \end{figure}

%   language specificity in humans using a behavioural metric, the `ABX' accuracy \citep{schatz_evaluating_2013}, which measures the ability to discriminate phones (Section XXXX). A) 
%   displays the ABX accuracy obtained by English and French participants on their native and non-native language. Error bars are standard error of the mean across phone pairs. \textbf{B)} ABX accuracy for the untrained, non-speech, French and English wav2vec 2.0 models, evaluated on the same datasets as the participants. C) Then, we compute the
  %In parallel, we collect the brain recordings of native subjects listening to stories in English, French or Mandarin. Subjects listen only to stories in their native language. 
  %Then, we evaluate the $R$ score obtained by each of these models for each subject independently. 
  %(i) the untrained model, (ii) the model trained on acoustic scenes, (iii) the model trained on a language different from their own, and (iv) the model trained on their own native language. We compute the corresponding brain scores. 
  %
%   \textbf{D)} %Voxels color-coded in black mark where the untrained model is significantly better than chance (p$<$ XXXXX). 
%   Purple voxels mark where the $R$ score of non-speech model outperforms the random model's (black); pink voxels mark where the $R$ score of non-native speech models outperform the non-speech models'; orange voxels mark where the $R$ score of native models (\emph{i.e.} models trained on the same language as the participant on whom it is compared) outperforms non-native models. These comparisons reveal where the sound-specific, speech-specific and language-specific representations learnt by wav2vec 2.0 are instantiated in the brain.
  %
  %if the model trained on acoustic scenes significantly outperforms the random model at predicting brain activity ($p<0.01$), `pink' if the model trained on non-native speech outperforms the acoustic model and `beige' if the native model outperforms the non-native model. 
  %
%   \textbf{B.} $R$ scores averaged across voxels for the untrained, acoustic, non-native and native models, in four brain regions typically associated with speech processing. The stars indicate a significant difference between the average brain scores of two models. %\textbf{C)} For the voxels where the non-native outperform the acoustic model, the difference in brain scores between the native and non-native models. 
%
%   \textbf{C)} We compare our four sets of self-supervised models with human behaviour using the `ABX` metric \citep{schatz_evaluating_2013}, which quantifies the ability to discriminate phonetic categories. The bar plots displays the accuracy of the models on $\approx$ 6,000 `ABX` triplets (testing 508 English and 524 French phone pairs). Non-speech and random models are evaluated on both French and English. Error bars are standard error of the mean across phone pairs. 
%   %
%   \textbf{D.} ABX accuracy obtained by human participants on the same datasets. French and English participants were evaluated on both French and English speech, \empH{i.e.} in their native or non-native language. Error bars are standard error of the mean across phone pairs. %C) and D) are restricted to French and English languages.
%   To do so, we use behavioural data from French and English-speaking participants tested on French and English stimuli. Statistics are computed over the phone pairs tested: ABX accuracy are first computed at the phone pair level and then averaged. The stars indicate a significant difference between the average ABX accuracy of two settings. 
  %
  %\textcolor{green}{TODO: add diagram for training regimes here?} 



% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.6\textwidth]{figures/Figure5_speechbrain.pdf}
%   \caption{\textbf{Discrimination scores for humans and models} We compare our self-supervised models with humans using behavioural data from French and English-speaking participants tested on French and English stimuli. Statistics are computed over the phone pairs tested: ABX accuracy are first computed at the phone pair level and then averaged. The stars indicate a significant difference between the average ABX accuracy of two settings. \textbf{A)} ABX accuracy (the bigger the better) for each training setting. \textbf{B)} ABX accuracy obtained by human participants.
%   }
%     \label{fig-ABX}
% \end{figure}


==> notes.tex <==

% 
% # Mapping cerveau deep nets. 
% # Mais pas plausible. (quantite de donnees, supervision, text, memory, attention span).
% 
% # Question: Here, we test whether a plausible model 

% 
% Est-ce qu'on a un mapping avec un modele plausible?
% Grande question: 
% Question: 
%
% # Enjeux: Si oui, une loi d'apprentissage qui suffit a expliquer l'organisation fonctionnelle du cerveau. 
% # => Conclusion speech: une loi qui sous-tend le traitement la parole 
% # => Conclusion neuro: a plausible candidate for speech processing in the brain.  modelisation fonctionnelle 
% # => Conclusion IA: non-supervise, bonne direction


% Charlotte : 
% (1) Speech processing in the brain: major unknowns -- the underlying representations, computations, architecture, learning objective. 

% (2) Limits of model-free approaches and limits of qualitative models of speech processing in the brain. 

% (3) Successes of deep-neural networks to replicate auditory behaviour

% (4 - option1) Q: deep neural networks as computational models of speech processing in the brain? *internal representations*. Trained with plausible learning objective, reasonable amount of data. 

% (4 option2) Recent computational models based on CNN and supervised methods (Kell) have evidenced converging internal representations between deep nets and the brain. Yet, implausibility: learning is unsupervised, large amount of data, convolution have limited time spans (). 

% (5) Here we propose a computational model of speech processing in the brain based on state-of-the-art neural networks, Wav2Vec2, trained with plausible amount of data, unsupervised objective and plausible attention span. 

% % Ideally: First, our model replicate human-like behaviour, achieving good performance at speech recognition tasks. 

% Second, we show that our model accurately predicts brain activity and outperforms previous approaches (MELs, task-optimized CNN). Furthermore, hierarchy ... . Critically, a similar model trained with annotated data and a supervised objective underperforms. Finally, we show how such a computational model enables us to study acoustic, speech, and language specific processing in the brain. 


% Structure of introduction should be
% General question: 
% - Speech = human uniqueness? No other animals, but deep nets start to provide remarkable models.

% Main challenges/question: 
% - understanding how the human brain processes speech?

% SOTA on these challenges
% Remaining challenge
% 1/ speech, not text
% 2/ no supervision
% 3/ plausible amount of training
% 4/ past research: limited amount of brain data, languages
% 
% Challenges left specific questions unanswered:
% - elements of convergence between self-supervised speech models and the brain
%    + converge to similar representations
%    + converge to similar hierarchy 
%    + better self-supervised than supervised: are linguists on the right track?
%    + language specific representations in the brain: does the brain simply recycle generic representations, or does it learn specific ones?
% Our approach:


